Data-Driven Stabilizing and Robust Control of Discrete-Time Linear Systems with Error in Variables

This work presents a sum-of-squares (SOS) based framework to perform data-driven stabilization and robust control tasks on discrete-time linear systems where the full-state observations are corrupted by L-infinity bounded input, measurement, and process noise (error in variable setting). Certificates of state-feedback superstability, quadratic stability or positive stability of all plants in a consistency set are provided by solving a feasibility program formed by polynomial nonnegativity constraints. Under mild compactness and data-collection assumptions, SOS tightenings in rising degree will converge to recover the true superstabilizing or positive stabilizing controller, with some conservatism introduced for quadratic stabilizability. The performance of this SOS method is improved through the application of a theorem of alternatives while retaining tightness, in which the unknown noise variables are eliminated from the consistency set description. This SOS feasibility method is extended to provide worst-case-optimal robust controllers under H2 control costs. The consistency set description may be broadened to include cases where the data and process are affected by a combination of L-infinity bounded measurement, process, and input noise.

==> sections/contributions.tex <==

The contributions of this paper are,
\begin{itemize}
    \item Formulation of stabilization  under \ac{EIV} as a polynomial optimization problem
    \item Application of \ac{SOS} methods to recover constant state-feedback (super, quadratic, positive) stabilizing controllers of all consistent plants with recorded data
    \item Simplification of \ac{SOS} programs by using a Theorem of Alternatives to eliminate affine-dependent noise variables
    \item Analysis of computational complexity of \ac{SOS} programs
\end{itemize}


Sections of this work were presented at the 61st Conference on Decision and Control \cite{miller2022eiv_short}. New content in this journal version as compared to the conference paper includes,
\begin{itemize}
    \item Extended superstabilization,  quadratic stabilization, and positive stabilization (the previous version only included superstability)
    \item Noting that a certificate function for superstability can be $\dx$-independent
     \item Derivation and application of the matrix Theorem of Alternatives ensuring Positive Definiteness
    \item Proofs of continuity, polynomial approximability, and convergence
     \item Worst-case-$H_2$ optimal control of consistent plants
    \item Further detail about the combination of measurement, input, and process noise    
 \end{itemize}

% \old{This paper proposes a convex, computationally tractable convex relaxation for  robust data driven control with  $\ell_\infty$ bounded measurement and process noise. Its main contributions are
%  \begin{enumerate}
%  \item To show that, in this scenario, robust superstabilizing  controllers can be designed by solving \ac{SOS}-based feasibility problems, which can be posed as \acp{SDP}. Robust stabilization is guaranteed by ensuring that all closed loop plants  consistent with the observed data are superstable. \item A theorem of alternatives reformulation that drastically reduces the number of variables involved and yields more tractable \acp{SDP} \cite{ben2015deriving}.
%  \end{enumerate}}

==> sections/hinf.tex <==
\subsection{H-infinity optimal control}
The controlled $H_\infty$ norm between $w \rightarrow z$ may be bounded by an \ac{LMI} 
from
%(8.8) of \cite{duan2013lmis},
Section 4.3.2 of \cite{caverly2019lmi},

\begin{prob}
The worst-case optimal $H_\infty$-norm of the system \eqref{eq:control_sys} over a set $(A, B)\in \pc$ is upper bounded by $\gamma \in \R_+$ if and only if  the below \ac{LMI} holds,
\begin{subequations}
 \label{eq:hinf_single}
\begin{align}
    \find_{\gamma,Y, S} \quad & \begin{bmatrix}
  Y & A Y - B S & E & \mathbf{0} \\
    \ast & Y & \mathbf{0} & Y C^T - S^T D_1^T \\
     \ast & \ast & \gamma I & D_2^T \\
     \ast & \ast& \ast& \gamma I
     \end{bmatrix} \in \psd_{++}^{2n+e+r}  \label{eq:hinf_single_lmi}\\
    &Y \in \psd^n, S \in \R^{m \times n}
\end{align}
\end{subequations}
The recovered control is $K = S Y^{-1}$.
\end{prob}

Algorithm \ref{alg:hinf} is the measurement-noise worst-case $H_\infty$ control problem, derived in a similar manner from \eqref{eq:hinf_single} as the $H_2$ algorithm \ref{alg:h2} originated from \eqref{eq:h2_single}.

\begin{algorithm}[h]
\caption{Worst-Case $H_\infty$ Program (full) \label{alg:hinf}}
\begin{algorithmic}
% \KwIn{$d, \ \delta, \ \dc, \ \epsilon, \ \Pi$}
\Procedure{$H_\infty$ Altern}{$d, \ \dc, \ \epsilon, E, \  C, \ D_1, \ D_2$}
% \KwOut{ $K, \ M$ (or Infeasibility)}
% $K \in \R^{n \times m}, \ M \in (\R[,B,\dx])^{n \times n}_{\leq 2d}$ \
Solve (or find infeasibility certificate):
% \begin{subequations}
\begin{align}
\min_{\gamma, Y, S} &  \qquad \gamma \label{eq:hinf_wsos} \\
% & \find_{\gamma,Y, S} \quad
&\begin{bmatrix}
  Y & A Y - B S & E & \mathbf{0} \\
    \ast & Y & \mathbf{0} & Y C^T - S^T D_1^T \\
     \ast & \ast & \gamma I & D_2^T \\
     \ast & \ast& \ast& \gamma I
     \end{bmatrix} \nonumber\\
    &\qquad \in \psd_{++}^{2n+e+r, \ \alt }[\Pi]_{\leq 2d} \nonumber\\
    &Y \in \psd^n, \ S \in \R^{m \times n}, \ \gamma \in \R_+ \nonumber
\end{align}
\Return $H_\infty = \gamma, \ K = S Y^{-1}$ (or Infeasibility)
\EndProcedure
% \end{subequations}
\end{algorithmic}
\end{algorithm}



% This section adapts the method from \cite{feron1992numerical} to perform worst-case \ac{LQR} control of all possible linear systems in the consistency set $\pc$.

% \subsection{LQR background}

% The discrete-time linear system model used in this section has a control input $u$, an exogenous input $w$, and a regulated output $z$ defined by matrices $Q \in \psd_{++}^n$ and $R \in \psd_{++}^m$,
% \begin{align}
%     x_{t+1} = Ax_t + Bu_t + w_t \label{eq:lqr_sys}\\
%     z_t = Q^{\frac{1}{2}}x_t + R^{\frac{1}{2}}u_t. \nonumber
% \end{align}

% Letting $G(j \omega)$ be the transfer function between $w \rightarrow z$, the \ac{LQR} problem finds a state-feedback controller $K$ with $u=Kx$ such that the $H_2$ norm $\norm{G}_2^2 = \int_{-\infty}^\infty$


% \urg{Talk about computational complexity? $H_2$ seems tolerable, but $H_\infty$ is a very large \ac{PMI}. 
% }

The H-infinity optimal control program in Algorithm \ref{alg:hinf} has one Scherer Psatz and no other PSD constraints. Letting $q_\infty = (2n+e+r)$ and $\nu_\infty = q_\infty (q_\infty+1)/2$, the sizes of PSD matrices in this Scherer Psatz are listed in \eqref{tab:hinf}.

\begin{table}[h]
    \centering
    % \begin{adjustbox}{width=0.48\textwidth}
    \begin{tabular}{ |c|c|c|c|c| }
 \hline
 Full & $q$ & $\sigma_0$ & $\sigma_i$ & $\mu_j$\\ \hline
 Number of Polynomials & 1 & 1 & $2nT$ & $2n(T-1)$ \\ \hline
 Full
 & $\R{\nu_\infty\binom{p_F + 2d}{2d}}$ 
 & $\psd_+q_\infty{\binom{p_F + d}{d}}$ 
 & $\psd_+q_\infty\binom{p_F + d - 1}{d- 1}$ 
 & $\R{\nu_\infty\binom{p_F + 2d-2}{2d-2}}$ \\ \hline
 Alternatives
 & $\R{\nu_\infty\binom{p_A + 2d}{2d}}$ 
 & $\psd_+q_\infty{\binom{p_A + d}{d}}$ 
 & $\psd_+ q_\infty\binom{p_A + d}{d}$ 
 & $\R{\nu_\infty\binom{p_A + 2d-1}{2d-1}}$ \\ \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Size of $H_\infty$ Control Method (Psatz)}
    \label{tab:hinf}
\end{table}

% \subsubsection{Chordal Sparsity}
The LMI constraint in \eqref{eq:hinf_single} contains chordal sparsity (refer to  \cite{vandenberghe2015chordal} for further detail). Labeling the column/row blocks of the matrix in \eqref{eq:hinf_single_lmi} as $(1,2,3,4)$, the symmetric \ac{PSD} matrix in \eqref{eq:hinf_single_lmi} has zero-entries in the specified locations of $(1,4)$ and $(2, 3)$. Agler's theorem \cite{agler1988positive} states that the sparse matrix in \eqref{eq:hinf_single_lmi} may be expressed as the sum of smaller \ac{PSD}. The two possible choices of chordal extensions of the aggregate sparsity pattern associated with the constraint in \eqref{eq:hinf_single_lmi} are the maximal cliques $\{(1,2,3), (2,3,4)\}$ and $\{(1,2,3), (1,2,4)\}$. Letting $X$ be the matrix from \eqref{eq:hinf_single_lmi} and $L_{123} \in \R^{(2n + e) \times (2n+e+r)}$ be the $0/1$ matrix associated with the projection $(x^1, x^2, w, z) \mapsto (x^1, x^2, w)$, there exists \ac{PSD} matrices 
\begin{subequations}
\begin{align}
    &X = L_{123}^T X_{123} L_{123} + L_{234}^T X_{234} L_{234} \\
    &X_{123} \in \psd_+^{2n+e}, \ X_{234} \in \psd_+^{n+e+r}.
\end{align}
\end{subequations}

A similar decomposition can take place for the selection of $\{(1,2,3), (1,2,4)\}$, yielding \ac{PSD} matrices of size $2n+e$ and $2n+r$.

This sparsity may be transferred the \ac{PMI} setting yielding sparse Scherer certificates by equation Theorem 2.4 of \cite{zheng2021pmi}. Convergence of Algorithm \ref{alg:hinf} to the true $H_\infty$ norm as the degree approaches infinity will hold under the assumption \ref{assum:compact} that $\Pi$ is Archimedean. The Gram matrix size associated with this sparse Psatz for the clique choices $\{(1,2,3), (2, 3, 4)\}$ are $\{(2n+e) \binom{p_A + d}{d}, (n+e+r) \binom{p_A + d}{d}\}$,  as compared to the size in table \ref{tab:hinf} of $\{(2n+e+r) \binom{p_A + d}{d}$.

Even with the application of sparsity, the SDP runtimes for modeling and execution of the Scherer Psatz constraints are extremely high. In this work, we reported experiments for the more tractable $H_2$ controller. 
% \urg{$H_2$ takes 40-80s for each example while $H_\infty$ takes around 1 hour for each example. Not sure if we should put it.}

% We note that the \ac{LMI} in 

==> sections/pos.tex <==
\section{Positive Systems Stabilization}
\label{sec:pos}

\urg{I'm positive!}

==> sections/sparse_altern.tex <==
% \section{Sparse Alternatives}
% \label{sec:sparse_altern}
% This section will present a sparse but conservative tightening of the Alternatives program in \eqref{eq:altern_sos}.

\subsection{Sparse Alternatives SOS}

The equality constraints in \eqref{eq:noise_bilinear} contain a grouping structure with respect to $(A, B)$. Groups $G_{i} = (A_{i, 1:n}, B_{i, 1:m})$ for $i=1..n$ may be defined by associating together variables in $(A, B)$ that share the same rows. Each scalar equality constraint \eqref{eq:noise_bilinear} only contains variables from one group as in,
\begin{equation}
 \hat{x}_{i, t+1} - \dx_{i, t+1} = \textstyle \sum_{j=1}^n A_{ij} (\hat{x}_{j, t} - \dx_{j, t}) + \sum_{j=1}^m B_{ij} u_{j, t}. \nonumber
\end{equation}

The matrix $M(A, B) \in \R[A,B]^{n, n}$ may be chosen to be the sum of group-$M$ matrices $M(A, B) = \sum_{i=1}^n M_i(G_i)$ for $M(G_i) \in \R[G_i]^{n \times n}$.
Letting $\Pi_i$ be an a-priori known Archimedean set containing $\pi^{G_i} \bpc$ for each $i=1..n$, the multipliers in \eqref{eq:altern_sos_zeta} and \eqref{eq:altern_sos_mu} may be chosen as,
\begin{subequations}
\begin{align}
    &\zeta^\pm_i(G_i) \in (\Sigma[\Pi_i]_{\leq 2d})^{n \times T} \label{eq:altern_sparse_zeta} &\forall i = 1..n  \\
    & \mu_i(G_i) \in (\R[G_i]_{\leq 2d-1})^{n \times (T-1)} \label{eq:altern_sparse_mu} & \forall i = 1..n.
\end{align}
\end{subequations}

The Psatz for $-Q$ in \eqref{eq:altern_sos_Q} may be certified as,
\begin{subequations}
\begin{align}
    &-Q(A, B; \zeta^\pm_{1:n}, \mu_{1:n}) = \textstyle \sum_{i=1}^n \sigma_i(G_i) \\
    & \sigma_i(G_i) \in \Sigma[\Pi_i]_{\leq 2d} & \forall i = 1..n, \label{eq:altern_sparse_sigma}
\end{align}
\end{subequations}
in a manner reminiscent to Correlative Sparsity \cite{waki2006sums}.

\subsection{Numerical Considerations}
This sparse formulation has a total of $n+m$ variables in any Gram matrix in \eqref{eq:altern_sparse_zeta} and \eqref{eq:altern_sparse_sigma}, yielding a maximum size of $\binom{n+m+d}{d}$. There are $2nT$ such Gram matrices in  \eqref{eq:altern_sparse_zeta} and $n$ maximal Gram matrices in \eqref{eq:altern_sparse_sigma}. This maximal size for Sparse Alternatives is far smaller than the Gram matrix sizes for either the Full or Alternatives program (as observed in Table \ref{tab:matrix_size_altern}), but conservatism is introduced as it is no longer guaranteed for the Sparse system to achieve convergence as $d$ increases.

% The maximum size of 
% The multipliers may chosen as 


% Defining the equality constraints as,
% \begin{equation}
    % h_{it} = 
% \end{equation}



==> sections/summary.tex <==

This paper is laid out as follows:
Section \ref{sec:preliminaries} introduces preliminaries such as acronym definitions, notation,  stability conditions for classes of linear systems, and \ac{SOS} methods. Section \ref{sec:full_method} creates a \ac{BSA} description of the consistency set of plants compatible with measurement-noise-corrupted data, and formulates \ac{SOS} algorithms to recover (super or quadratic) stabilizing controllers. Section \ref{sec:altern} reduces the computational complexity of these \ac{SOS} programs by eliminating the affine-dependent measurement noise variables through a Theorem of Alternatives. 
Section \ref{sec:optimal_control} applies the Full and Alternative methods to synthesize worst-case-optimal controllers for systems under measurement noise. 
Section \ref{sec:complexity} quantifies this reduction in computational complexity by analyzing the size and multiplicities of \ac{PSD} matrices involved in these \ac{SOS} methods.
Section \ref{sec:all_noise} extends the previously presents \ac{SOS} formulations to problems with measurement, input, and process noise. 
Section \ref{sec:examples} demonstrates the \ac{SOS} stabilizing algorithms on a set of examples. 
% Section \ref{sec:extensions} extends the \ac{SOS} framework to cases including varying noise sets, non-uniform sampling times, and switched systems stabilization (with a known switching sequence). 
Section \ref{sec:conclusion} concludes the paper.
Appendix \ref{app:sos} reviews details of \ac{SOS} methods with scalar nonnegativity and matrix positive-semidefiniteness constraints.  
Appendix \ref{app:continuity} proves that multiplier functions for the Alternatives program may be chosen to be continuous. Appendix \ref{app:polynomial_sw} builds on this continuity result and proves that the multiplier functions may also be chosen to be symmetric-matrix-valued polynomials.
% \old{
% % Section \ref{sec:sparse_altern} formulates a sparse tightening to the Alternatives program with reduced computational cost. 
% Section \ref{sec:examples} presents numerical experiments validating this method. Section \ref{sec:extensions} details extensions such as the varying noise sets, input noise, and the combination of process and measurement noise.
% % \urg{could cut down or swap out any of these. Non-uniform sampling time and switched systems (with tracking) are both available and have not been implemented yet.}
% The paper is concluded in Section \ref{sec:conclusion}. 
% }
% An extended version of this paper is available at \urg{Arxiv Link} and includes \urg{[content]}.
